Generalized multifractality at spin quantum Hall transition

Generalized multifractality characterizes scaling of eigenstate observables at Anderson-localization critical points. We explore generalized multifractality in 2D systems, with the main focus on the spin quantum Hall (SQH) transition in superconductors of symmetry class C. Relations and differences with the conventional integer quantum Hall (IQH) transition are also studied. Using the field-theoretical formalism of non-linear sigma-model, we derive the pure-scaling operators representing generalizing multifractality and then "translate" them to the language of eigenstate observables. Performing numerical simulations on network models for SQH and IQH transitions, we confirm the analytical predictions for scaling observables and determine the corresponding exponents. Remarkably, the generalized-multifractality exponents at the SQH critical point strongly violate the generalized parabolicity of the spectrum, which implies violation of the local conformal invariance at this critical point.

==> Iwasawa.tex <==
In this section we focus on two constructions based on the Iwasawa decomposition. Let us briefly  outline basic steps in this approach. We begin with the Cartan decomposition
\begin{align}
\mfg= \mfk \oplus \mfp
\label{Cartan-decomposition-real}
\end{align}
of the real Lie algebra $\mfg= \text{so}^*(4n)$ into a maximal compact subalgebra $\mfk= \text{u}(2n)$ and the complementary subspace $\mfp$. The parts of the real Cartan decomposition satisfy the  commutation relations similar to those in the complex case \eqref{comm-rel-Cartan-complex}
\begin{align}
[\mfk, \mfk] &\subseteq \mfk,
&
[\mfk, \mfp] &\subseteq \mfp,
&
[\mfp, \mfp] &\subseteq \mfk.
\label{comm-rel-Cartan-real}
\end{align}

Then we choose a maximal Abelian subspace $\mfa \subset \mfp$
and consider the adjoint action of elements of $\mfa$ on $\text{so}^*(4n)$. The eigenvectors $E_\alpha$ of this action satisfy
\begin{align}
[H, E_\alpha] = \alpha(H) E_\alpha
\end{align}
and are called {\it restricted} root vectors, and the eigenvalues $\alpha$ are called restricted roots. The dimension $m_\alpha$ of the restricted root space
\begin{align}
\mfg_\alpha = \text{span}\, \{E_\alpha\}
\end{align}
is called the multiplicity of the restricted root $\alpha$, and can be bigger that 1. Restricted roots are linear functions on $\mfa$, and lie in the space $\mfa^*$ dual to $\mfa$. In the present context both $\mfa$ and $\mfa^*$ have dimension $n$. Basis elements in the space $\mfa^*$ are denoted by $x_i$ ($i = 1,\ldots, n$) and will be specified later.

A system of positive restricted roots is defined by choosing some hyperplane through the origin of $\mfa^*$ which divides $\mfa^*$ in two halves, and then defining one of these halves as positive. The Weyl vector $\rho$  is defined as the half-sum of positive restricted roots accounting for their multiplicities:
\begin{align}
\rho = \sum_{\alpha > 0} m_\alpha \alpha = \sum_{i=1}^{n} c_i x_i.
\end{align}
The components $c_i$ of the Weyl vector will be found later, see Eq. \eqref{Weyl-vector-components}. Positive restricted roots generate the nilpotent Lie algebra
\begin{align}
\mfn = \sum_{\alpha > 0} \mfg_\alpha.
\end{align}
The Iwasawa decomposition
\begin{align}
\mfg= \mfk\oplus \mfa \oplus \mfn
\label{Iwasawa-decomposition-algebra}
\end{align}
replaces the root-space decomposition \eqref{root-space-decpomposition} in the real setting. Similar to Eq. \eqref{n+decomposition} we have
\begin{align}
\mfn = \mfp\oplus (\mfn \cap \mfk).
\end{align}

Exponentiation of Eq. \eqref{Iwasawa-decomposition-algebra} gives the global form of the Iwasawa decomposition
\begin{align}
G = NAK,
\label{Iwasawa-decomposition-group}
\end{align}
which allows us to represent any element $g \in G$ in the form $g = nak$, with $n \in N = e^\mfn$, $a \in A = e^\mfa$, and $k \in K = e^{\mfk}$. This factorization is unique once the system of positive restricted roots is fixed, and provides a very useful parametrization of the target space $G/K$. An element $a \in A$ is fully specified by $n$ real numbers $x_i(\ln a)$, which play the role of radial coordinates on $G/K$. For simplicity, we will denote these radial coordinates simply by $x_i$. Thus $x_i$ may now have two different meanings: either its original meaning as a basis element in $\mfa^*$, or the new one as an $N$-radial function $x_i(\ln a)$ on $G/K$. It should be clear from the context which of the two meanings is being used.

Using the radial coordinates, the joint $N$-radial eigenfunctions of the Laplace-Casimir operators on $G/K$ take a very simple exponential form
\begin{align}
\varphi_\mu(Q) = e^{(\rho + \mu)(\ln a)},
\label{plane-wave-1}
\end{align}
where $a$ is the $a$-factor in the Iwasawa decomposition of $g$ in $Q = g \Lambda g^{-1}$, and
\begin{align}
\mu = \sum_{i=1}^{n} \mu_i x_i
\end{align}
is a weight vector in $\mfa^*$. We will also use the notation
\begin{align}
q_i = -(\mu_i + c_i)/2,
\end{align}
in which the exponential functions \eqref{plane-wave-1} become
\begin{align}
\varphi_\mu \equiv \varphi_{(q_1,q_2,\ldots,q_n)} = \exp \Big(-2 \sum_{i=1}^{n} q_i x_i \Big).
\label{plane-wave-2}
\end{align}

To construct the exponential $N$-radial eigenfunctions explicitly as combinations of matrix elements of $Q$, we can proceed in two directions. The first one, explained in detail in Section \ref{sec:N-radial-functions}, uses the key fact that there exists a choice of basis in which elements of $\mfa$ and $a \in A$ are diagonal matrices, while elements of $\mfn$ are strictly upper triangular, and elements $n \in N$ are upper triangular with units on the diagonal. This has immediate consequences for the matrix $Q \Lambda$: since elements of $K$ commute with $\Lambda$, the Iwasawa decomposition $g = nak$ leads to $Q \Lambda = n a^2 \Lambda n^{-1} \Lambda$, which is a product of upper triangular, diagonal, and a lower triangular matrices. In this form the principal minors of the $AA$ block of $Q \Lambda$ are simply products of diagonal elements of $a^2$, which are exponentials of radial coordinates $x_i$ on $G/K$. These minors are basic $N$-radial spherical functions on $G/K$ which can be raised to arbitrary powers and multiplied to produce the most general exponential functions \eqref{plane-wave-1}. A great advantage of this construction is that is directly gives the general positive scaling operators that can be raised to arbitrary powers and satisfy the Abelian fusion rules.

An alternative way to construct positive scaling operators is similar to the HWV method of Section \ref{sec:hwv}, except that now we construct restricted HWVs, that is, functions $\phi_\lambda(Q)$ that satisfy
\begin{align}
\widehat{X} \phi_\lambda &= 0,
&& \text{for all } X \in \mfn,
\label{RHWV-definition-1}
\\
\widehat{H} \phi_\lambda &= \lambda(H) \phi_\lambda,
&& \text{for all } H \in \mfa.
\label{RHWV-definition-2}
\end{align}
The construction involves polynomials of the $\mu$-functions \eqref{mu-function} with $Y \in \mfp$, see Section \ref{sec:rhwv}.



Let us discuss how the two constructions based on the Iwasawa decomposition are related to each other. $N$-radial functions $f(Q)$ on $G/K$ by definition have the invariance property
\begin{align}
f(n Q n^{-1}) = f(Q) && \forall n \in N.
\label{N-invariance}
\end{align}
Any such function is automatically a restricted HWV. Indeed, if $X \in \mfn$ is an element of the Lie algebra of $N$, then
%\begin{align}
$(\widehat{X} f)(Q)
%= \frac{d}{dt}\Big|_{t=0} f\big(e^{-tX} Q\, e^{tX})
= 0$,
%\end{align}
since the expression under the $t$ derivative in Eq. \eqref{X-hat-action} does not depend on $t$ by the invariance \eqref{N-invariance}.


\subsection{Cartan decomposition and generators}

The group $\text{SO}^*(4n)$ is connected, so all its elements can be written as $g = e^Z$, where $Z$ are elements of the Lie algebra $\text{so}^*(4n)$. These satisfy the infinitesimal versions of Eqs. \eqref{SO-star-definition-Knapp}:
\begin{align}
Z^\dagger \Sigma_{30} + \Sigma_{30} Z &= 0,
&
Z^T \Sigma_{10} + \Sigma_{10} Z &= 0,
\label{so-star-definition-Knapp}
\end{align}
In terms of the Lie algebra involutions $\theta_i$ related to the group involutions \eqref{group-involutions}
\begin{align}
\theta_i(Z) &\equiv - \Sigma_{i0} Z^T \Sigma_{i0},
\label{Lie-algebra-involutions}
\end{align}
constraints on $Z$ can be written as
\begin{align}
\theta_3(Z) &= Z^*,
&
\theta_1(Z) &= Z.
\label{so-star-definition-Knapp-involutions}
\end{align}
If we write the Lie algebra elements $Z$ as block-matrices in the AR space, the constraints \eqref{so-star-definition-Knapp} imply
\begin{align}
Z &= \begin{pmatrix} A & B \\ - B^* & A^* \end{pmatrix},
&
A^\dagger&= - A,
&
B^T & - B.
\label{so-star-Knapp}
\end{align}

The Cartan involution that determines the Cartan decomposition $\text{so}^*(4n) = \mfk+ \mfp$ into even and odd subspaces is $\theta_2$. It acts on generators $Z$ as
\begin{align}
\theta_2(Z) &= - \Sigma_{20} Z^T \Sigma_{20}
= \begin{pmatrix} A & -B \\ B^* & A^* \end{pmatrix}.
\end{align}
This gives us a very explicit description of the Cartan decomposition:
\begin{align}
\mfk&= \left\{ \begin{pmatrix} A & 0 \\ 0 & A^* \end{pmatrix},
\quad
A^\dagger = - A \right\},
&
\mfp&= \left\{ \begin{pmatrix} 0 & B \\ -B^* & 0 \end{pmatrix},
\quad
B^T = - B \right\}.
\label{Cartan-spaces}
\end{align}
As expected, the subalgebra $\mfk= \text{u}(2n)$, the Lie algebra of $K = \text{U}(2n)$, the maximal compact subgroup in $G = \text{SO}^*(4n)$.

Now we separate the real and imaginary parts in Eq. \eqref{Cartan-spaces}:
\begin{align}
\mfk&= \left\{ \begin{pmatrix} A_1 + iA_2 & 0 \\ 0 & A_1 - iA_2 \end{pmatrix},
\begin{array}{l} A_1^T = - A_1 \\ A_2^T = A_2 \end{array}
\right\},
&
\mfp&= \left\{ \begin{pmatrix} 0 & B_1 + i B_2 \\ -B_1 + i B_2 & 0 \end{pmatrix},
\begin{array}{l} B_1^T = - B_1 \\ B_2^T = - B_2 \end{array}
\right\}.
\end{align}
These forms allow us to write the generators of the two subsets in terms of tensors in the space \eqref{tensor-product-space}. For elements in $\mfk$, the first factor should be diagonal, so it is either $I_2$ or $i\sigma_3$. For the first choice ($I_2$), the other two tensor factors should produce a real anti-symmetric matrix, which can be done choosing one of the factors to be a symmetric matrix, and the other an anti-symmetric matrix. Likewise, for the second choice ($i\sigma_3$) we need the other two factors to produce a real symmetric matrix, so the factors can be either simultaneously symmetric or anti-symmetric. Introducing a short-hand notation for the symmetric and anti-symmetric combinations of matrix units in the replica space
\begin{align}
E^+_{ij} & = E_{ij} + E_{ji},
& i &\leqslant j,
& \frac{n(n+1)}{2} \quad \text{total},
\\
E^-_{ij} & = E_{ij} - E_{ji},
& i &< j,
& \frac{n(n-1)}{2} \quad \text{total},
\end{align}
we get the following eight groups of generators:
\begin{align}
X^{00}_{ij} &\equiv \sigma_0 \otimes \sigma_0 \otimes E^-_{ij},
&
X^{01}_{ij} &\equiv \sigma_0 \otimes \sigma_1 \otimes E^-_{ij},
&
X^{02}_{ij} &\equiv \sigma_0 \otimes i\sigma_2 \otimes E^+_{ij},
&
X^{03}_{ij} &\equiv \sigma_0 \otimes \sigma_3 \otimes E^-_{ij},
\nonumber \\
X^{30}_{ij} &\equiv i\sigma_3 \otimes \sigma_0 \otimes E^+_{ij},
&
X^{31}_{ij} &\equiv i\sigma_3 \otimes \sigma_1 \otimes E^+_{ij},
&
X^{32}_{ij} &\equiv i\sigma_3 \otimes i\sigma_2 \otimes E^-_{ij},
&
X^{33}_{ij} &\equiv i\sigma_3 \otimes \sigma_3 \otimes E^+_{ij}.
\label{k-generators}
\end{align}
The total number of generators here is $4n^2 = (2n)^2$, the dimension of $\mfk= \text{u}(2n)$, as it should be.

Similarly, for the elements in $\mfp$, the first factor should be either
$i \sigma_1$ or $i \sigma_2$, and for either of these choices the remaining two factors should give a real anti-symmetric matrix. This gives the following eight groups of generators:
\begin{align}
Y^{10}_{ij} &= i\sigma_1 \otimes \sigma_0 \otimes E^-_{ij},
&
Y^{11}_{ij} &= i\sigma_1 \otimes \sigma_1 \otimes E^-_{ij},
&
Y^{12}_{ij} &= i\sigma_1 \otimes i\sigma_2 \otimes E^+_{ij},
&
Y^{13}_{ij} &= i\sigma_1 \otimes \sigma_3 \otimes E^-_{ij},
\nonumber \\
Y^{20}_{ij} &= i\sigma_2 \otimes \sigma_0 \otimes E^-_{ij},
&
Y^{21}_{ij} &= i\sigma_2 \otimes \sigma_1 \otimes E^-_{ij},
&
Y^{22}_{ij} &= i\sigma_2 \otimes i\sigma_2 \otimes E^+_{ij},
&
Y^{23}_{ij} &= i\sigma_2 \otimes \sigma_3 \otimes E^-_{ij}.
\label{p-generators}
\end{align}
The total number of these generators is $4n^2 - 2n = 2n(2n-1)$, which is the dimension of the space $\mfp$.


\subsection{Iwasawa decomposition}


We choose the following set of Hermitian matrices as the maximal Abelian subspace $\mfa \subset \mfp$:
\begin{align}
\mfa &= \text{span}\left\{ H_k = i\sigma_2 \otimes i\sigma_2 \otimes E_{kk}
= Y_{22,kk}/2, \quad k = 1,\ldots, n \right\}.
\end{align}
A generic element $H \in \mfa$ is
%\begin{align}
$H = \sum_{k=1}^n h_k H_k$.
%\end{align}
We define the basis in the dual space $\mfa^*$ as elements $x_i$ such that $x_i(H) = h_i$. These elements will later play the role of the radial coordinates on the coset $\text{SO}^*(4n)/\text{U}(2n)$.

To find restricted roots and restricted root vectors, we need to find the commutators of $H$ with the generators \eqref{k-generators} and \eqref{p-generators}. We need both sets since the commutation relations \eqref{comm-rel-Cartan-real} imply that
\begin{align}
[\mfa, \mfk] &\subset \mfp,
&
[\mfa, \mfp] &\subset \mfk,
\end{align}
so the eigenvectors of the adjoint action of $\mfa$ can only be linear combinations of generators from both sets.

Straightforward computations show that the system of restricted roots consists of roots of normal length $\pm x_i \pm x_j$ ($i \neq j$) with multiplicity 4, and long roots $\pm 2x_j$ with multiplicity 1. This is the root system $C_n$ in the usual Cartan notation. The set of positive restricted roots can be chosen as (multiplicities shown in brackets)
\begin{align}
\alpha_{ij} &\equiv x_i - x_j, \quad i < j \quad (4),
&
\beta_{ij} &\equiv x_i + x_j, \quad i < j \quad (4),
&
\gamma_i &\equiv 2x_i \quad (1).
\end{align}
The Weyl vector (the half-sum of positive restricted roots accounting for their multiplicities) is
\begin{align}
\rho &= (4n - 3)x_1 + (4n-7)x_2 +\ldots+ 5x_{n-1} + x_n
= \sum_{j=1}^{n} c_j x_j,
&
c_j &= 4n + 1 - 4j.
\end{align}
In the replica limit $n \to 0$ the components of the Weyl vector become
\begin{align}
c_j = 1 - 4j.
\label{Weyl-vector-components}
\end{align}
The positive restricted root vectors corresponding to the $\alpha$,
$\beta$, and $\gamma$ roots are
\begin{align}
E_{\alpha_{ij}}^{(1)} &= X^{00}_{ij} + Y^{22}_{ij},
%= \sigma_0 \otimes \sigma_0 \otimes E^-_{ij}
%+ i\sigma_2 \otimes i\sigma_2 \otimes E^+_{ij},
%\nonumber \\
&
E_{\alpha_{ij}}^{(2)} &= X^{02}_{ij} - Y^{20}_{ij},
%= \sigma_0 \otimes i\sigma_2 \otimes E^+_{ij}
%- i\sigma_2 \otimes \sigma_0 \otimes E^-_{ij},
%\nonumber \\
&
E_{\alpha_{ij}}^{(3)} &= X^{31}_{ij} - Y^{13}_{ij},
%= i\sigma_3 \otimes \sigma_1 \otimes E^+_{ij}
%- i\sigma_1 \otimes \sigma_3 \otimes E^-_{ij},
%\nonumber \\
&
E_{\alpha_{ij}}^{(4)} &= X^{33}_{ij} + Y^{11}_{ij},
%= i\sigma_3 \otimes \sigma_3 \otimes E^+_{ij}
%+ i\sigma_1 \otimes \sigma_1 \otimes E^-_{ij},
%\nonumber \\
\\
E_{\beta_{ij}}^{(1)} &= X^{01}_{ij} + Y^{23}_{ij},
%= \sigma_0 \otimes \sigma_1 \otimes E^-_{ij}
%+ i\sigma_2 \otimes \sigma_3 \otimes E^-_{ij},
%\nonumber \\
&
E_{\beta_{ij}}^{(2)} &= X^{03}_{ij} - Y^{21}_{ij},
%= \sigma_0 \otimes \sigma_3 \otimes E^-_{ij}
%- i\sigma_2 \otimes \sigma_1 \otimes E^-_{ij},
%\nonumber \\
&
E_{\beta_{ij}}^{(3)} &= X^{30}_{ij} - Y^{12}_{ij},
%= i\sigma_3 \otimes \sigma_0 \otimes E^+_{ij}
%- i\sigma_1 \otimes i\sigma_2 \otimes E^+_{ij},
%\nonumber \\
&
E_{\beta_{ij}}^{(4)} &= X^{32}_{ij} + Y^{10}_{ij},
%= i\sigma_3 \otimes i\sigma_2 \otimes E^-_{ij}
%+ i\sigma_1 \otimes \sigma_0 \otimes E^-_{ij},
%\nonumber \\
\\
E_{\gamma_i} &= X^{30}_{ii} - Y^{12}_{ii}.
%= i\sigma_3 \otimes \sigma_0 \otimes E_{ii}
%- i\sigma_1 \otimes i\sigma_2 \otimes E_{ii}.
\end{align}
As we mentioned above, these vectors generate a nilpotent subalgebra $\mfn$, and we get the resulting Iwasawa decomposition \eqref{Iwasawa-decomposition-algebra}.

\subsection{Real scaling operators as $N$-radial functions}
\label{sec:N-radial-functions}

In this section we perform a unitary transformation of basis in the space \eqref{tensor-product-space} designed to bring the generators of $\mfa$ into a diagonal form. There are infinitely many such transformations, and the one we choose has an additional useful property that the resulting positive restricted root vectors are also upper-triangular in the RA space. This is achieved with the help of the unitary matrix
\begin{align}
U &=
%\frac{1}{\sqrt{2}}
%\begin{pmatrix} 1 & 0 & 0 & i \\ 0 & i & 1 & 0 \\
% 0 & -i & -1 & 0 \\ 1 & 0 & 0 & -i \end{pmatrix}
%=
\frac{1}{\sqrt{2}} (\sigma_0 \otimes E_{11} + \sigma_1 \otimes E_{12} - \sigma_2 \otimes E_{21} - i \sigma_3 \otimes E_{22}) \otimes I_n,
\label{U-Iwasawa}
\end{align}
where we used the $2 \times 2$ matrix units $E_{ij}$ in the spin space. While this is not a single tensor product in the RA and spin spaces, conjugation with this matrix,
\begin{align}
T(A) \equiv U A U^{-1},
\label{T-rotation}
\end{align}
keeps such single products in the basis of $\mfa$:
\begin{align}
T(H_k) = \sigma_3 \otimes \sigma_0 \otimes E_{kk},
\end{align}
in the the saddle point
\begin{align}
T(\Lambda) = - \Sigma_{12},
\label{T-Lambda}
\end{align}
as well as in the restricted root vectors:
\begin{align}
T(E_{\alpha_{ij}}^{(1)}) &= \sigma_0 \otimes \sigma_0 \otimes E^-_{ij}
+ \sigma_3 \otimes \sigma_0 \otimes E^+_{ij}
= 2 E_{11} \otimes \sigma_0 \otimes E_{ij}
- 2 E_{22} \otimes \sigma_0 \otimes E_{ji},
\nonumber \\
T(E_{\alpha_{ij}}^{(2)}) &= i\sigma_3 \otimes \sigma_1 \otimes E^+_{ij}
+ i\sigma_0 \otimes \sigma_1 \otimes E^-_{ij}
= 2 i E_{11} \otimes \sigma_1 \otimes E_{ij}
- 2 i E_{22} \otimes \sigma_1 \otimes E_{ji},
\nonumber \\
T(E_{\alpha_{ij}}^{(3)}) &= -i \sigma_0 \otimes \sigma_2 \otimes E^+_{ij} - i\sigma_3 \otimes \sigma_2 \otimes E^-_{ij}
= -2 i E_{11}\otimes \sigma_2 \otimes E_{ij}
+ 2 i E_{22} \otimes \sigma_2 \otimes E_{ji},
\nonumber \\
T(E_{\alpha_{ij}}^{(4)}) &= i\sigma_3 \otimes \sigma_3 \otimes E^+_{ij}
+ i\sigma_0 \otimes \sigma_3 \otimes E^-_{ij}
= 2 i E_{11} \otimes \sigma_3 \otimes E_{ij}
+ 2 i E_{22} \otimes \sigma_3 \otimes E_{ji},
\nonumber \\
T(E_{\beta_{ij}}^{(1)}) &= \sigma_1 \otimes \sigma_0 \otimes E^-_{ij}
+ i\sigma_2 \otimes \sigma_0 \otimes E^-_{ij}
=  2 E_{12} \otimes \sigma_0 \otimes E^-_{ij},
\nonumber \\
T(E_{\beta_{ij}}^{(2)}) &= -\sigma_2 \otimes \sigma_1 \otimes E^-_{ij}
+ i\sigma_1 \otimes \sigma_1 \otimes E^-_{ij}
= 2i E_{12} \otimes \sigma_1 \otimes E^-_{ij},
\nonumber \\
T(E_{\beta_{ij}}^{(3)}) &= -i\sigma_1 \otimes \sigma_2 \otimes E^+_{ij}
+ \sigma_2 \otimes i\sigma_2 \otimes E^+_{ij}
= - 2 i E_{12} \otimes \sigma_2 \otimes E^+_{ij},
\nonumber \\
T(E_{\beta_{ij}}^{(4)}) &= -\sigma_2 \otimes \sigma_3 \otimes E^-_{ij} + i\sigma_1 \otimes \sigma_3 \otimes E^-_{ij}
= 2 i E_{12} \otimes \sigma_3 \otimes E^-_{ij}
\nonumber \\
T(E_{\gamma_i}) &= -2i\sigma_1 \otimes \sigma_2 \otimes E_{ii}
+ 2 \sigma_2 \otimes i\sigma_2 \otimes E_{ii}
= - 4 i E_{12} \otimes \sigma_2 \otimes E_{ii}.
\end{align}
As claimed, the structure in the RA space is upper triangular: in the first factor we have either $E_{11}$ and $E_{22}$ or $E_{12}$.

We can visualize the restricted root vectors for $n=3$ as a schematic matrix diagram by indicating the matrix positions where various generators have non-zero entries. For brevity we write $\gamma_i\equiv E_{\gamma_i}$, $\alpha^{(i)}\equiv E^{(i)}_{\alpha_{kl}}$, $\beta^{(i)}\equiv E^{(i)}_{\beta_{kl}}$ with indices suppressed since they can be inferred from the matrix grid (uncolored cells have zero entries):
\begin{align}
T(E) = \left(\begin{array}{ccc|ccc|ccc|ccc}
\caplus x_1 & \calphare& \calphare \alpha^{(14)}  & & \calphaim & \calphaim \alpha^{(23)}  & & \cbetare & \cbetare \beta^{(14)} & \cgamma \gamma_1 & \cbetaim & \cbetaim \beta^{(23)}\\
 & \caplus x_2 & \calphare &  & &\calphaim  &\cbetare &   & \cbetare  & \cbetaim & \cgamma \gamma_2 & \cbetaim \\
 & & \caplus x_3  & & &  &\cbetare \beta^{(14)} & \cbetare & & \cbetaim \beta^{(23)} & \cbetaim & \cgamma \gamma_3\\
\hline
& \calphaim & \calphaim \alpha^{(23)}  & \caplus x_1 & \calphare & \calphare \alpha^{(14)}  & \cgamma  \gamma_1 & \cbetaim & \cbetaim \beta^{(23)} & & \cbetare & \cbetare \beta^{(14)}\\
& & \calphaim & & \caplus x_2 & \calphare & \cbetaim & \cgamma \gamma_2 & \cbetaim & \cbetare & & \cbetare \\
& &   & & & \caplus x_3  & \cbetaim \beta^{(23)} & \cbetaim & \cgamma \gamma_3  & \cbetare \beta^{(14)} & \cbetare &  \\
\hline
& &  & & &  & \caminus -x_1 & &  & & &\\
& & &  & & & \calphare & \caminus -x_2 & &\calphaim & & \\
& &  & & &   &\calphare \alpha^{(14)} & \calphare & \caminus -x_3  &\calphaim\alpha^{(23)} & \calphaim & \\
\hline
 & &  & & &  & & &  & \caminus -x_1 & & \\
 & &  & & &  &\calphaim & &  & \calphare & \caminus -x_2 & \\
 & &  & & &  &\calphaim \alpha^{(23)} & \calphaim &   & \calphare \alpha^{(14)} & \calphare & \caminus -x_3 \\
\end{array}\right).
\label{matrix-rrvs}
\end{align}
This matrix can be made upper triangular by an additional permutation $\pi$ of the basis vectors that can be described explicitly as follows: for $i \in 1, \ldots, n$, we have
\begin{align}
\pi(i) &= 2i-1,
&
\pi(n+i) &= 2i,
&
\pi(2n+i) &= 4n + 2 - 2i,
&
\pi(3n+i) &= 4n + 1 - 2i.
\label{permutation-pi}
\end{align}
This permutation re-sorts the diagonal entries of the matrix \eqref{matrix-rrvs} as follows:
\begin{align}
x_1, \ldots, x_n, x_1, \ldots, x_n, -x_1, \ldots, -x_n, -x_1, \ldots, -x_n
&& \to &&
x_1, x_1, \ldots, x_n, x_n, -x_n, -x_n, \ldots, -x_1, -x_1.
\end{align}
The permutation matrix $P_\pi$ that corresponds to $\pi$ has the matrix elements $(P_\pi)_{ij} = \delta_{\pi(i), j}$, and can be used to permute rows and columns of a matrix $M$ as follows:
\begin{align}
(P_\pi M)_{ij} &= M_{\pi(i), j},
&
(M P_\pi^{-1})_{ij} &= M_{i,\pi(j)}.
\end{align}
Then we can see that the conjugation of the matrix \eqref{matrix-rrvs} by $P_\pi$ makes it fully upper-triangular. Using the notation
\begin{align}
\tilde{M} \equiv P_\pi T(M) P_\pi^{-1},
\label{tilde-M}
\end{align}
for transformed matrices, we have
\begin{align}
\tilde{E} = \left(\begin{array}{cccccc|cccccc}
\caplus x_1 & & \calphare & \calphaim & \calphare & \calphaim &   \cbetare & \cbetaim & \cbetare & \cbetaim &   & \cgamma \gamma_1\\
& \caplus x_1 & \calphaim & \calphare & \calphaim & \calphare &   \cbetaim & \cbetare & \cbetaim &  \cbetare & \cgamma \gamma_1 &  \\
& & \caplus x_2 & & \calphare & \calphaim &   \cbetare & \cbetaim & & \cgamma \gamma_2 &  \cbetare & \cbetaim \\
& & & \caplus x_2 & \calphaim & \calphare &    \cbetaim  & \cbetare & \cgamma \gamma_2 &  & \cbetaim & \cbetare\\
& & & & \caplus x_3 & &    & \cgamma \gamma_3  & \cbetare & \cbetaim & \cbetare & \cbetaim \\
& & & & & \caplus x_3 &   \cgamma \gamma_3 &  & \cbetaim & \cbetare & \cbetaim &\cbetare\\
\hline
& & &  & & &  \caminus -x_3 & & \calphare & \calphaim & \calphare & \calphaim\\
& & &  & & &  & \caminus -x_3 & \calphaim & \calphare & \calphaim & \calphare\\
& & &  & & &  & & \caminus -x_2 & & \calphare & \calphaim\\
& & &  & & &  & & &\caminus -x_2 & \calphaim& \calphare\\
& & &  & & &  & &  &  & \caminus -x_1 & \\
& & &  & & &  & & &  & & \caminus -x_1 \\
\end{array}\right).
\label{matrix-rrvs-triangular}
\end{align}
In the final basis the elements of $\mfa$ are diagonal matrices, while elements of $\mfn$ are strictly upper triangular.

Let us exploit consequences of the Iwasawa decomposition of $G$ and the transformation $T$ for the sigma model field $Q$. First of all, in the original basis where $\Lambda = \Sigma_{30}$ we write $g = nak$ with $n \in N$, $a \in A$, and $k \in K$, and then
\begin{align}
\mathcal{Q} &\equiv Q \Lambda = nak \Lambda k^{-1} a^{-1} n^{-1} \Lambda
= n a^2 \Lambda n^{-1} \Lambda.
\end{align}
Here we used $k \Lambda k^{-1} = \Lambda$ and $a \Lambda a^{-1} = a^2
\Lambda$, which is a special case of the first condition in Eq. \eqref{SO-star-definition-Knapp} for a Hermitian matrix $a \in G$. Now we perform the transformation $T$, Eq. \eqref{T-rotation}, as well as the permutation $P_\pi$. Using the notation \eqref{tilde-M}, we get
\begin{align}
\tilde{\mathcal{Q}} = \tilde{n} \tilde{a}^2 \tilde{\Lambda} \tilde{n}^{-1} \tilde{\Lambda}.
%= \tilde{n} \tilde{a}^2 P_\pi \Sigma_{12} P_\pi^{-1} \tilde{n}^{-1} P_\pi \Sigma_{12} P_\pi^{-1}.
\end{align}
Using Eqs. \eqref{T-Lambda} and \eqref{permutation-pi}, we can compute the matrix
\begin{align}
\tilde{\Lambda} = - P_\pi \Sigma_{12} P_\pi^{-1}
= - \sigma_1 \otimes \sigma_2 \otimes \mathcal{I}_n,
\end{align}
where $\mathcal{I}_n$ is the $n \times n$ matrix with units on the ``anti-diagonal'', that is, $(\mathcal{I}_n)_{ij} = \delta_{i, n + 1 - j}$.

As should be clear from the previous discussion, the matrices $\tilde{n}$ and $\tilde{n}^{-1}$ are upper-triangular with units on the diagonals, while $\tilde{a}$ is diagonal:
\begin{align}
\tilde{a} = \text{diag} (e^{x_1}, e^{x_1}, \ldots, e^{x_n}, e^{x_n}, e^{-x_n}, e^{-x_n},\ldots, e^{-x_1}, e^{-x_1}).
\end{align}
Conjugation by $\tilde{\Lambda}$ converts $\tilde{n}^{-1}$ into $\tilde{\Lambda} \tilde{n}^{-1} \tilde{\Lambda}$ which is {\it lower-triangular} with units on the diagonal. This results in the following structure of the $AA$ block of the matrix $\tilde{\mathcal{Q}}$:
\begin{align}
\tilde{\mathcal{Q}}_{AA} =
\begin{pmatrix} 1 & * & \ldots & * & * \\
0 & 1 & \ldots & * & * \\
\vdots & \vdots & \ddots & \vdots & \vdots\\
0 & 0 & \ldots & 1 & * \\
0 & 0 & \ldots & 0 & 1 \end{pmatrix}
\begin{pmatrix} e^{-2x_n} & 0 & \ldots & 0 & 0 \\
0 & e^{-2x_n} & \ldots & 0 & 0 \\
\vdots & \vdots & \ddots & \vdots &\vdots \\
0 & 0 & \ldots & e^{-2x_1} & 0 \\
0 & 0 & \ldots & 0 & e^{-2x_1} \end{pmatrix}
\begin{pmatrix} 1 & 0 &\ldots &0 &0 \\
* & 1 & \ldots & 0 & 0 \\
\vdots & \vdots & \ddots & \vdots & \vdots \\
* & * & \ldots & 1 & 0 \\ * & * & \ldots & * & 1 \end{pmatrix}.
\label{Q-tilde-AA}
\end{align}
Determinants of the lower-right $2m \times 2m$ submatrices of $\tilde{\mathcal{Q}}_{AA}$ give the basic positive $N$-radial eigenfunctions
\begin{align}
d_{2m} = \prod_{i = 1}^{m} e^{-4x_i}
= \exp \Big(- 4 \sum_{i=1}^{m} x_i \Big).
\label{basic-d-2m}
\end{align}
We can form the most general $N$-radial eigenfunctions as products
\begin{align}
\varphi_{(q_1,\ldots,q_n)} = d_2^{(q_1 - q_2)/2} d_4^{(q_2 - q_3)/2}
\ldots d_{2(n-1)}^{(q_{n-1} - q_n)/2} d_{2n}^{q_n/2},
\label{d-product}
\end{align}
where we may take the $q_i$ to be arbitrary complex numbers. It is easy to see that the product \eqref{d-product} is the same as the exponential eigenfunction \eqref{plane-wave-2}, while the basic function $d_{2m}$ is $\varphi_{(2,2,\ldots)}$ with $m$ twos in the subscript.

Notice that the doubling of the diagonal entries $e^{-2x_i}$ for each $i$ in Eq. \eqref{Q-tilde-AA} compelled us to take determinants of sub-matrices of even size and raise the resulting functions to powers written as $(q_i - q_{i+1})/2$. This is very similar to the appearance of minors of even size in Section \ref{sec:HWV-so-4n-C}. Those minors were of an anti-symmetric matrix, and thus were squares of Pfaffians, see Eq. \eqref{p-m-expansion}. In the Iwasawa formalism it is also possible to obtain directly the ``Pfaffian'' solutions $\varphi_{(1,1,\ldots)}$. Pfaffians can be defined only for anti-symmetric matrices, so we need to look at transformation properties of various matrices under transposition. For group elements $g$ this property in given in the second equation in \eqref{SO-star-definition-Knapp}. We can use this equation to derive the following consequence:
\begin{align}
T(g)^T &= (U \Sigma_{10} U^T)^{-1} T(g)^{-1} (U \Sigma_{10} U^T).
\end{align}
%Here
%\begin{align}
%U^T = \frac{1}{\sqrt{2}} (\sigma_0 \otimes E_{11} + \sigma_1 \otimes E_{21} + \sigma_2 \otimes E_{12} - i \sigma_3 \otimes E_{22}) \otimes I_n,
%\end{align}
%and a 
A simple computation shows that $U \Sigma_{10} U^T = \Sigma_{10}$. Thus the rotated matrix $T(g)$ satisfies the same second equation in \eqref{SO-star-definition-Knapp}:
\begin{align}
T(g)^{-1} = \Sigma_{10} T(g)^T \Sigma_{10}.
\end{align}

Let us now look at
\begin{align}
T(Q \Lambda) = T(g) T(\Lambda) T(g)^{-1} T(\Lambda)
= T(g) \Sigma_{12} \Sigma_{10} T(g)^T \Sigma_{10} \Sigma_{12}
= T(g) \Sigma_{02} T(g)^T \Sigma_{02},
\end{align}
which means that $T(Q \Lambda) \Sigma_{02}$ is anti-symmetric. Now we can employ the Iwasawa decomposition $T(g) = T(n) T(a) T(k)$ and drop the last factor, since in $T(Q\Lambda)$ the group element $g$ enters only in the product $g \Lambda g^{-1}$, and $k$ commutes with $\Lambda$:
\begin{align}
T(Q \Lambda) \Sigma_{02}
= T(n) T(a) \Sigma_{02} [T(n) T(a)]^T.
\end{align}
Next, we restrict everything to the $AA$ block using the upper triangular structure of $T(n)$ and the diagonal nature of $T(a)$ in the RA space, see Eq. \eqref{matrix-rrvs}. In this block $\Sigma_{02,AA} = \sigma_2 \otimes I_n$, and we have
\begin{align}
T(Q \Lambda)_{AA} (\sigma_2 \otimes I_n)
= T(n)_{AA} T(a)_{AA} (\sigma_2 \otimes I_n) [T(n)_{AA} T(a)_{AA}]^T.
\end{align}
We can use the property of the Pfaffians $\text{Pf} \, (M A M^T) = \det(M) \, \text{Pf} \, A$, where $A$ is anti-symmetric and $M$ arbitrary, to obtain
\begin{align}
\text{Pf} \, [T(Q \Lambda)_{AA} (\sigma_2 \otimes I_n)]
= \det[T(n)_{AA}] \det[T(a)_{AA}] \, \text{Pf} \, (\sigma_2 \otimes I_n).
\end{align}
Since the determinant is basis-independent, we have
\begin{align}
\det[T(n)_{AA}] &= \det[\tilde{n}_{AA}] = 1,
&
\det[T(a)_{AA}] &= \det[\tilde{a}_{AA}] = \prod_{i=1}^{n} e^{-2x_i}.
\end{align}
Finally, we get the Pfaffian $N$-radial functions
\begin{align}
p_n \equiv \varphi_{(1,1,\ldots)} = \exp \Big(-2 \sum_{i=1}^{n} x_i \Big)
= \frac{\text{Pf} \, [T(Q \Lambda)_{AA} (\sigma_2 \otimes I_n)]}{\text{Pf} \, (\sigma_2 \otimes I_n)} \label{eq:nradial}.
\end{align}
This can be done for arbitrary number of replicas $n$, so we get all basic Pfaffians this way, and the most general $N$-radial functions
\begin{align}
\varphi_{(q_1,\ldots,q_n)} = p_1^{q_1 - q_2} p_2^{q_2 - q_3}
\ldots p_{n-1}^{q_{n-1} - q_n} p_n^{q_n}.
\label{p-product}
\end{align}


\subsection{Real scaling operators as restricted HWVs}
\label{sec:rhwv}

{\bf Discuss basis independence of the algebraic structure, but basis dependence of the resulting functions on $G/K$}

